Learning Illumination Patterns for Coded Diffraction Phase Retrieval

Signal recovery from nonlinear measurements involves solving an iterative optimization problem. In this paper, we present a framework to optimize the sensing parameters to improve the quality of the signal recovered by the given iterative method. In particular, we learn illumination patterns to recover signals from coded diffraction patterns using a fixed-cost alternating minimization-based phase retrieval method. Coded diffraction phase retrieval is a physically realistic system in which the signal is first modulated by a sequence of codes before the sensor records its Fourier amplitude. We represent the phase retrieval method as an unrolled network with a fixed number of layers and minimize the recovery error by optimizing over the measurement parameters. Since the number of iterations/layers are fixed, the recovery incurs a fixed cost. We present extensive simulation results on a variety of datasets under different conditions and a comparison with existing methods. Our results demonstrate that the proposed method provides near-perfect reconstruction using patterns learned with a small number of training images. Our proposed method provides significant improvements over existing methods both in terms of accuracy and speed.

==> definitions.tex <==
\usepackage{graphicx}
\usepackage{amsmath,amsfonts,amsthm,amssymb,xspace,bm, verbatim,dsfont}
\usepackage{url,algorithm,algpseudocode}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{cleveref}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{positioning,plotmarks,calc}
\usepackage{bbm}
\usepackage{todonotes}
\usepackage{subfig}
\usepackage{pgfplots}

% \usepackage{subcaption}

%% Theorems, Lemmas, Proofs, Definitions %%
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}

%% Notes %%
\theoremstyle{definition}
\newcommand{\note}[1]{\marginpar{\tiny *note in TeX*}}
%% Operators %%

%Probability%
\DeclareMathOperator*{\pr}{\mathsf{Pr}}
\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
\DeclareMathOperator*{\ex}{\mathbb{E}}
\newcommand{\expec}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\normal}{\mathcal{N}(0,1)}
\newcommand{\gauss}{\mathcal{N}}

%Real and Complex spaces
\newcommand{\rn}{\mathbb{R}^n}
\newcommand{\rnn}{\mathbb{R}^{n \times n}}
\newcommand{\rmm}{\mathbb{R}^{m \times m}}
\newcommand{\rmn}{\mathbb{R}^{m \times n}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}

%Identity and ones
\newcommand{\eye}{\mathbb{I}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\ones}{\mathbbm{1}}

%Vectors and Matrices%
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}

%Matrix operations - Trace, Rank, Norms, Inner products
\newcommand{\iprod}[2]{\left\langle #1, #2 \right\rangle} 
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\phase}[1]{\mathrm{Ph}\left(#1\right)}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\imag}[1]{\textrm{Im}\left(#1\right)}

%\newcommand{\norm}[1]{{\left\lVert{#1}\right\rVert}}
\newcommand{\frob}[1]{\left\| {#1} \right\|_\text{F}}
\newcommand{\zeronorm}[1]{\left\| {#1} \right\|_0}
\newcommand{\onenorm}[1]{\left\| {#1} \right\|_1}
\newcommand{\twonorm}[1]{\left\| {#1} \right\|_2}
\newcommand{\infnorm}[1]{\left\| {#1} \right\|_{\infty}}

\newcommand{\sign}[1]{\operatorname{sign}\left(#1\right)}
\newcommand{\Tr}{\operatorname{Tr}}
\DeclareMathOperator{\trace}{Tr}

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\dist}[2]{\|#1-#2\|_2}
\newcommand{\distop}[2]{\mathrm{dist}\left(#1,#2\right)}

%Sets
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\card}[1]{\operatorname{card}(#1)}
\newcommand{\trunc}[1]{\operatorname{trunc}(#1)}

%Complexity
\newcommand{\order}[1]{\mathcal{O}\left({#1}\right)}
\newcommand{\ordereps}[1]{\mathcal{O}_{\epsilon}\left({#1}\right)}
%Brackets
\newcommand{\rbrak}[1]{\left(#1\right)}
\newcommand{\sbrak}[1]{\left[#1\right]}
\newcommand{\cbrak}[1]{\left\{#1\right\}}
\newcommand{\sqfr}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\frsq}[2]{\frac{#1}{\sqrt{#2}}}

%Paper-specific variables%
%\newcommand{\eps}{\epsilon}
\newcommand{\y}{\vect{y}}
\newcommand{\e}{\vect{e}}
\newcommand{\z}{\vect{z}}
\newcommand{\w}{\vect{w}}
\newcommand{\uu}{\vect{u}}
\newcommand{\rr}{\vect{r}}
\newcommand{\vv}{\vect{v}}
\newcommand{\zhat}{\hat{\z}}
\newcommand{\xo}{\vect{x^*}}
\newcommand{\xin}{\vect{x^0}}
%\newcommand{\x}{\vect{x}}
\newcommand{\xt}{\x^t}
\newcommand{\xtplus}{\x^{t+1}}
\newcommand{\xplus}{\x^+}
\newcommand{\xtilde}{\vect{\widetilde{x}}}
\newcommand{\xSmin}{\x_{S_{-}}^*}
\newcommand{\xSpls}{{\x_{S_{+}}^*}}
\newcommand{\xSbmin}{\x_{S_{b-}}^*}
\newcommand{\xSbpls}{{\x_{S_{b+}}^*}}
\newcommand{\xShat}{{\x_{\hat{S}}^*}}
\newcommand{\xSbhat}{{\x_{\hat{S_b}}^*}}
\newcommand{\xS}{\x_{S}^*}
\newcommand{\ai}{\vect{a}_i}
\newcommand{\aiS}{{\ai_{S}}}
\newcommand{\aiShat}{{\ai}_{\hat{S}}}
\newcommand{\aiSmin}{\ai_{S_{-}}}
\newcommand{\aiSpls}{\ai_{S_{+}}}
\renewcommand{\P}{\mat{P}}
\newcommand{\p}{\vect{p}}
\newcommand{\h}{\vect{h}}
\newcommand{\A}{\mat{A}}
\newcommand{\D}{\mat{D}}
\newcommand{\M}{\mat{M}}
\newcommand{\U}{\mat{U}}
\newcommand{\subspaces}{{\mathcal{M}}}


%\newcommand{\red}[1]{\textcolor{red}{#1}}
%\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}
%
%\newcommand*{\AddNote}[4]{%
%	\begin{tikzpicture}[overlay, remember picture]
%	\draw [decoration={brace,amplitude=0.5em},decorate,ultra thick,red]
%	($(#3)!(#1.north)!($(#3)-(0,1)$)$) --  
%	($(#3)!(#2.south)!($(#3)-(0,1)$)$)
%	node [align=center, text width=2.5cm, pos=0.5, anchor=west] {#4};
%	\end{tikzpicture}
%}%

\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\mA}{\ensuremath{\mathbf A}}
\newcommand{\mB}{\ensuremath{\mathbf B}}
\newcommand{\mE}{\ensuremath{\mathbf E}}
\newcommand{\mF}{\ensuremath{\mathbf F}}
\newcommand{\mG}{\ensuremath{\mathbf G}}
\newcommand{\mL}{\ensuremath{\mathbf L}}
\newcommand{\mM}{\ensuremath{\mathbf M}}
\newcommand{\mQ}{\ensuremath{\mathbf Q}}
\newcommand{\mR}{\ensuremath{\mathbf R}}
\newcommand{\mS}{\ensuremath{\mathbf S}}
\newcommand{\mT}{\ensuremath{\mathbf T}}
\newcommand{\mU}{\ensuremath{\mathbf U}}
\newcommand{\mV}{\ensuremath{\mathbf V}}
\newcommand{\mW}{\ensuremath{\mathbf W}}
\newcommand{\mX}{\ensuremath{\mathbf X}}
\newcommand{\mY}{\ensuremath{\mathbf Y}}
\newcommand{\mZ}{\ensuremath{\mathbf Z}}
\newcommand{\ve}{\ensuremath{\mathbf e}}
\newcommand{\va}{\ensuremath{\mathbf a}}
\newcommand{\vb}{\ensuremath{\mathbf b}}
\newcommand{\vc}{\ensuremath{\mathbf c}}
\newcommand{\vf}{\ensuremath{\mathbf f}}
\newcommand{\vg}{\ensuremath{\mathbf g}}
\newcommand{\vh}{\ensuremath{\mathbf h}}
\newcommand{\vp}{\ensuremath{\mathbf p}}
\newcommand{\vr}{\ensuremath{\mathbf r}}
\newcommand{\vs}{\ensuremath{\mathbf s}}
\newcommand{\vu}{\ensuremath{\mathbf u}}
%\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\vw}{\ensuremath{\mathbf w}}
\newcommand{\vx}{\ensuremath{\mathbf x}}
\newcommand{\vy}{\ensuremath{\mathbf y}}
\newcommand{\vz}{\ensuremath{\mathbf z}}
\newcommand{\vpsi}{\ensuremath{\mathbf \psi}}
\newcommand{\vphi}{\ensuremath{\mathbf \phi}}
\newcommand{\ct}{\ensuremath{\widetilde{c}}}
\newcommand{\setT}{\ensuremath{\mathcal T}}
\newcommand{\proj}{\ensuremath{\mathcal P}}
\newcommand{\rf}[1]{\ensuremath{{\mathbf \phi}_{#1}}}
\newcommand{\af}[1]{\ensuremath{\underline{\mathbf f}_{#1}}}
\newcommand{\ru}[1]{\ensuremath{{\mathbf u}_{#1}}}
\newcommand{\qa}[1]{\ensuremath{\hat{a}_{#1}}}
\newcommand{\comp}[2]{\ensuremath{c_{#1,#2}}}
\newcommand{\resid}[2]{\ensuremath{\vr_{#1,#2}}}
\newcommand{\cerr}[2]{\ensuremath{\ct_{#1,#2}}}
\newcommand{\vsW}{\ensuremath{\mathcal{W}}}
\newcommand{\vsS}{\ensuremath{\mathcal{S}}}
\newcommand{\vsH}{\ensuremath{\mathcal{H}}}
\newcommand{\opF}{\ensuremath{\mathbf{F}}}
\newcommand{\piF}{\ensuremath{\mathbf{F}^\dagger}}
\newcommand{\adjF}{\ensuremath{\mathbf{F}^*}}
\newcommand{\Epsilon}{\ensuremath{\mathcal{E}}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\SD}{\ensuremath{\Sigma\Delta}}
\newcommand{\MMSE}{\ensuremath{\mbox{MMSE}}}
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\dvec}{\bf vec}
%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\diag}{diag}
%\newcommand{\supp}[1]{\ensuremath{\operatorname{supp}\left(#1\right)}}
\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}\left(#1\right)}}
\newcommand{\nullsp}[1]{\ensuremath{\operatorname{null}(#1)}}
\newcommand{\range}[1]{\ensuremath{\operatorname{range}(#1)}}
\renewcommand{\dim}[1]{\ensuremath{\operatorname{dim}(#1)}}
\newcommand{\spanof}[1]{\ensuremath{\operatorname{span}\{#1\}}}
\newcommand{\rankof}[1]{\ensuremath{\operatorname{rank}\{#1\}}}
%\newcommand{\qed}{\framebox{}}
\newtheorem{Theorem}{Theorem}
\newtheorem{Definition}{Definition}
\newtheorem{Lemma}{Lemma}
\newcommand{\PBnote}[1]{{\em [**PB:{#1}]}}
\newcommand{\Salnote}[1]{{\em [**SAL:{#1}]}}


\newcommand{\field}[1]{\mathbb{#1}}                                   % Topological sets
\newcommand{\prn}[1]{\left(#1\right)}                                 % Parenthetical
\newcommand{\Prn}[1]{\left[#1\right]}                                 % Parenthetical 2
\newcommand{\clog}[1]{\textnormal{Log}\left(#1\right)}                % Complex Logarithm
\newcommand{\cfn}[2]{#1\left(#2\right)}                               % Continuous function
\newcommand{\dfn}[2]{#1\left[#2\right]}                               % Discrete function
\newcommand{\dff}[2]{\displaystyle\frac{d#1}{d#2}}                    % Differential (fraction form)
\newcommand{\dfe}[2]{\displaystyle\frac{d}{d#2}\left(#1\right)}       % Differential (expression form)
\newcommand{\pdff}[2]{\displaystyle\frac{\partial #1}{\partial #2}}   % Partial Differential (fraction form)
\newcommand{\pdfe}[2]{\displaystyle\frac{\partial}{\partial #2}#1}    % Partial Differential (expression form)
\newcommand{\pdo}[1]{\displaystyle\frac{\partial}{\partial #1}}       % Partial Differential Operator
%dfrac:   \newcommand{\nfrac}[2]{\displaystyle\frac{#1}{#2}}                    % Display Fraction
\newcommand{\dlim}[2]{\displaystyle\lim_{#1}\left(#2\right)}          % Display Limit
\newcommand{\dint}[3]{\displaystyle\int_{#1}^{#2}{#3}}                % Display Integral
\newcommand{\dsum}[3]{\displaystyle\sum_{#1}^{#2}{#3}}                % Display Sum
\newcommand{\centerup}[1]{\begin{center}#1\end{center}}               % Center text
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}                         % Horizontal line
%\newcommand{\abs}[1]{\left|#1\right|}                                 % Absolute value
\newcommand{\elone}[1]{\left\|#1\right\|_1}                           % L-1 Norm
\newcommand{\eltwo}[1]{\left\|#1\right\|_2}                           % L-2 Norm
\newcommand{\elinf}[1]{\left\|#1\right\|_\infty}                      % L-infinity Norm
\newcommand{\fro}[1]{\left\|#1\right\|_{fro}}                         % Frobenius Norm
%\newcommand{\norm}[1]{\left\|#1\right\|}                              % Norm
\renewcommand{\labelenumi}{(\alph{enumi})}                            % To get enumerate to display letters
\newcommand{\ip}[1]{\langle{#1}\rangle}																 % Inner Product
\newcommand{\sarray}[1]{\begin{array}{l}#1\end{array}}								 % simple array
\newcommand{\sarrayc}[1]{\begin{array}{c}#1\end{array}}								 % simple array (center)
\newcommand{\darray}[1]{\begin{array}{ll}#1\end{array}}								 % double array
\newcommand{\darraycl}[1]{\begin{array}{cl}#1\end{array}}							 % double array (center,left)
\newcommand{\res}[1]{\centerup{\framebox{#1}}}												 % Important result (centered and boxed)
\newcommand{\amatrix}[1]{\begin{bmatrix}#1\end{bmatrix}}							 % matrix (bmatrix)
\newcommand{\minim}[2]{\underset{#1}{\min}{#2}}												 % minimize
\newcommand{\maxim}[2]{\underset{#1}{\max}{#2}}												 % maximize
%\newcommand{\sign}[1]{\mathrm{sign}{\left(#1\right)}}									 % sign function
%
% Theorems, Lemmas, Proposition...
%
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{definition}{Definition}[section]
%
% LCA Symbols
%
\newcommand{\G}{\Gamma}
\newcommand{\Gc}{\Gamma^c}
\newcommand{\g}{\gamma}
\newcommand{\PP}{\Phi_{\Gamma}^T\Phi_{\Gamma}}
\newcommand{\PcP}{\Phi_{\Gamma^c}^T\Phi_{\Gamma}}
%
% Custom Trig functions
%
\newcommand{\cosine}[1]{\mathbf{\cos}\left(#1\right)}
\newcommand{\sine}[1]{\mathbf{\sin}\left(#1\right)}
\newcommand{\cosinep}[2]{\mathbf{\cos}^{#2}\left(#1\right)}
\newcommand{\sinep}[2]{\mathbf{\sin}^{#2}\left(#1\right)}
\newcommand{\tangent}[1]{\tan\left(#1\right)}
\newcommand{\cosecant}[1]{\csc\left(#1\right)}
\newcommand{\secant}[1]{\sec\left(#1\right)}
\newcommand{\cotangent}[1]{\cot\left(#1\right)}
\newcommand{\arctangent}[1]{\tan^{-1}\left(#1\right)}
\newcommand{\arcsine}[1]{\arcsin\left(#1\right)}
\newcommand{\arccosine}[1]{\arccos\left(#1\right)}
\newcommand{\hypsine}[1]{\sinh\left(#1\right)}
\newcommand{\hypcosine}[1]{\cosh\left(#1\right)}
\newcommand{\hyptangent}[1]{\tanh\left(#1\right)}
\newcommand{\atanq}[2]{\arctangent{\gfrac{#1}{#2}}}
%
% Custom tabbing
%
\newcommand{\etab}{\ \ \ \ }
\newcommand{\dnl}{\newline\newline}                                  % Double newline
%
% Probability Functions
%
\newcommand{\expc}[1]{E\left[#1\right]}	                             % Expectation
\newcommand{\expco}[2]{E\left[\left.#1\right|#2\right]}              % Conditional Expectation
\newcommand{\exps}[2]{E_{#1}\left[#2\right]}                         % Expectation with subscript
\newcommand{\var}[1]{\texttt{var}\func{#1}}		                       % Variance
\newcommand{\vars}[2]{\texttt{var}_{#1}\func{#2}}                    % Variance with subscript
\newcommand{\cov}[1]{\texttt{cov}\func{#1}}		                       % Covariance
\newcommand{\pdf}[2]{\mkfunc{f_{#1}}{#2}}                            % Probability Distribution Function
%\newcommand{\pr}[1]{Pr\func{#1}} 						                         % Probability
%
% Probability Distributions
%
\newcommand{\gaussian}[1]{\dfrac{1}{\sqrt{2\pi\sigma_{#1}^2}}e^{-\frac{\prn{#1-\mu_{#1}}^2}{2\sigma_{#1}^2}}}
%
% Figure
%
\newcommand{\fig}[4]{\begin{figure}
\begin{center}
\includegraphics[width=#1]{#2}
\caption{#3}
\label{fig:#4}
\end{center}
\end{figure}}
%
\newcommand{\figh}[4]{\begin{figure}[h]
\begin{center}
\includegraphics[width=#1]{#2}
\caption{#3}
\label{fig:#4}
\end{center}
\end{figure}}

